Singularities of matrix semicircles

Let $S=\sum_{i=1}^r A_i\otimes s_i$ be a matrix semicircular element, with Hermitian coefficients $A_i\in M_n(\mathbb{C})$ and free standard semicircular generators $s_i$. Its scalar spectral density $f$ is governed, through Speicher's equation (a matrix Dyson equation), by the completely positive covariance map $\eta_S(X)=\sum_i A_iXA_i$. We treat the singular regime, where the pencil $\sum_i A_i x_i$ is full but not semisimple and $f$ is unbounded at the origin, in contrast to the bounded real-analytic density of the regular case. We prove three results. (i) The leading singularity exponent at $0$ is invariant under congruence $A_i\mapsto bA_ib^{*}$ of the pencil ($b$ invertible), and more generally under symmetric scaling of the covariance map. (ii) For binary elements ($r=2$) we obtain a complete classification: in Lancaster-Rodman canonical form every indecomposable cell is of one of three types, and $f(x)\sim c|x|^{-(n^*-1)/(n^*+1)}$ as $x\to0$ with an explicit constant $c$, where the exponent depends only on the size of the largest Jordan block (the effective chain length $n^*$) and not on the coupling. With (i) and the direct-sum behaviour, this classifies all full binary Hermitian pencils. (iii) The spectral classification is strictly coarser than the algebraic one: a Type III cell of size $2m$ with non-real $\beta$ and the direct sum of two Type II cells of size $m$ with parameter $|\beta|$ have identical scalar densities, yet their covariance maps are not symmetrically scalable; the scalar spectrum cannot detect the phase of $\beta$. Each type calls for a different method: a reduction of Speicher's equation to an autonomous discrete Painlev\'e I (McMillan) map (Type I), a Lyapunov-Schmidt reduction at the branch point (Type II), and a gauge reduction by a diagonal unitary (Type III).

==> mathPreambuleReport.tex <==
\usepackage{amssymb, amsfonts, amsmath, amsthm,mathtools}
\usepackage{mathrsfs} %Nice calligraphic font
%%\usepackage{enumerate} %-- this is simpler package
\usepackage{enumitem} %-- this gives a bit more freedom
\usepackage[dvipsnames]{xcolor}
\usepackage{wrapfig}
\usepackage{mathdots}
\usepackage{tikz-cd}

%\input Rothdn.fd
%\renewcommand*\initfamily{\usefont{U}{Rothdn}{xl}{n}}
%
\usepackage{bbm}
\newcommand{\1}{\mathbbm{1}} % Blackboard bold 1 for indicator function.


\RequirePackage{graphicx}
\RequirePackage{hyperref}
\RequirePackage[small,bf]{caption}
\RequirePackage{actuarialangle}


\renewcommand{\baselinestretch}{1.2}
\renewcommand{\emph}{\textbf}


%%%%%%%%%%%%%%%%%%%%%%%
%%Modify Table of Contents
%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{titletoc}


%%%%%%%%%%%
%A shortcut for alignment environment and for equations
%%%%%%%%%%%
\newcommand{\bal}[1]{\begin{align*}#1\end{align*}}
\newcommand{\beq}[1]{\begin{equation}#1\end{equation}}

%A shortcut for matrices
\newcommand{\bmatr}[1]{\begin{bmatrix}#1\end{bmatrix}}


%%%colors
\newcommand{\blue}{\color{blue}}
\newcommand{\red}{\color{red}}
\newcommand{\orange}{\color{orange}}
\newcommand{\cyan}{\color{cyan}}
\newcommand{\magenta}{\color{magenta}}
\newcommand{\green}{\color{green}}


\newcommand{\bi}{\mathbf{i}} %quaternion units
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}


\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\let\C\bC
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\N}{\mathbb{N}} %natural numbers
\newcommand{\bP}{\mathbb{P}}
\renewcommand{\P}{\bP} %another version of probability
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\Z}{\mathbb{Z}} %ring of integers


\newcommand{\HS}{\mathrm{HS}}

\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Corr}{\mathrm{Corr}}
\newcommand{\Wg}{\mathrm{Wg}}
\newcommand{\Var}{\mathbb{V}\mathrm{ar}}
\newcommand{\Ad}{\mathrm{Ad}}
\newcommand{\Trace}{\mathrm{Tr}}
\newcommand{\eps}{\varepsilon}
\newcommand{\range}{\mathrm{Range\,}}
\newcommand{\im}{\mathrm{Range\,}}
\newcommand{\ran}{\mathrm{Range\,}}
\newcommand{\Id}{I}
\newcommand{\GL}{\mathrm{GL}}
\newcommand{\Fix}{\operatorname{Fix}}
\newcommand{\ext}{\operatorname{ext}}


%\renewcommand{\phi}{\varphi}
\renewcommand{\bar}[1]{\overline{#1}}
\renewcommand{\Re}{\mathrm{Re}\,} %redefining Re and Im commands
\renewcommand{\Im}{\mathrm{Im}\,}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Herm}{\mathrm{Herm}}

\newcommand{\nat}{\mathrm{nat}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\chain}{\mathrm{ch}}
\newcommand{\frakR}{\mathfrak R}
\newcommand{\fR}{\mathfrak R}


\newcommand{\df}{\stackrel{{{\mathrm{def}}}}{=}}
\newcommand{\func}[1]{\mathrm{#1}}
\newcommand\stack[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}
\newcommand{\QED}{\hfill $\square$}  

\newcommand{\scP}[2]{\left\langle #1, #2\right\rangle} %scalar product
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}

\newcommand{\TypeI}{\ensuremath{\mathrm{Type\ I}}}
\newcommand{\TypeII}{\ensuremath{\mathrm{Type\ II}}}
\newcommand{\TypeIII}{\ensuremath{\mathrm{Type\ III}}}

\newcommand{\ovln}[1]{\overline{#1}}
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\oc}[1]{\overset{\circ}{#1}} %Puts a circle on the argument. 

\newcommand{\Cl}{\mathcal{C}\ell}
\newcommand{\rn}{\mathrm{rn}}
\DeclareMathOperator{\blk}{bk} %number of blocks in a partition
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Det}{Det}
\DeclareMathOperator{\ord}{ord} %order of a function
\DeclareMathOperator{\supp}{supp} %support of a measure
\DeclareMathOperator{\diag}{diag} %diagonal matrix
\DeclareMathOperator{\plim}{plim} %probability limit
\DeclareMathOperator{\Capa}{Cap} %capacity
%\DeclareMathOperator{\Fix}{Fix} %set of fixed points  
\DeclareMathOperator{\lhull}{span} % linear span (hull) of a set of vectors. 
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\BL}{BL} %Banach limit
\DeclareMathOperator{\DS}{DS}

\newcommand{\Ker}{\operatorname{Ker}}
\newcommand{\spanop}{\operatorname{span}}


%%%%%%%%%%%%%%%%%%%%%%%%%%
%Various shortcuts for convergences
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pwcv{\stackrel{\scriptscriptstyle p.w.}{\longrightarrow}}     % pointwize convergence
\def\ascv{\stackrel{\scriptscriptstyle a.s.}{\longrightarrow}}     % almost sure convergence
\def\pcv{\stackrel{\scriptscriptstyle \P}{\longrightarrow}}        % convergence in P
\def\ltcv{\stackrel{\scriptscriptstyle\LL^2}{\longrightarrow}}      % L2 convergnece
\def\lpcv{\stackrel{\scriptscriptstyle\LL^p}{\longrightarrow}}      % Lp convergnece
\def\dcv{\stackrel{\scriptscriptstyle d}{\longrightarrow}}         % convergence in d
\def\wcv{\stackrel{\scriptscriptstyle w}{\longrightarrow}}         % weak
\def\deq{\stackrel{\scriptscriptstyle d}{=}}			   % equal in d
\def\toinf{\to \infty}
\def\ci{\perp\!\!\!\perp}  % conditional independence
\newcommand{\convpoint}{\stackrel{p.w.}{\longrightarrow}}
\newcommand{\conv}{\rightarrow}
\newcommand{\xto}{\xrightarrow}
\newcommand{\dashfrom}{\dashleftarrow}
\newcommand{\dashto}{\dashrightarrow}
\def\pto{\stackrel{p}{\longrightarrow}} %convergence in probability


%\newcommand{\B}{\BB} %another version for Borel field
\newcommand{\fL}{\mathrm{L}}   %upright L for functional spaces
\newcommand{\ZZ}{\mathcal{Z}} %Center of an algebra
\newcommand{\XX}{\mathcal{X}} %Determinantal field
\newcommand{\bT}{\mathbb{T}} %Torus
\newcommand{\TT}{\mathcal{T}} %Graph of tilings
\newcommand{\calS}{\mathcal{S}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\RR}{\mathcal{R}} %Another form of R-transform.
\newcommand{\QQ}{\mathcal{Q}}
\newcommand{\PP}{\mathcal{P}}
\newcommand{\MM}{\mathcal{M}} %right module of quaternion polynomials
\newcommand{\VV}{\mathcal{V}} %standard left module for Temperley-Lieb algebra.
\newcommand{\LL}{\mathcal{L}} %Normalized bracket polynomial
\newcommand{\KK}{\mathcal{K}} %rescaled kernel
\newcommand{\II}{\mathcal{I}} %interface, or interval
\newcommand{\HH}{\mathcal{H}} %sigma-field 
\newcommand{\GG}{\mathcal{G}} %another sigma-field 
\newcommand{\FF}{\mathcal F}
\newcommand{\DD}{\mathcal D}
\newcommand{\CC}{\mathcal C}
\newcommand{\BB}{\mathcal B}
\renewcommand{\AA}{\mathcal A}

\newcommand{\PD}{\mathcal{PD}}

\newcommand{\cB}{\mathcal B}
\newcommand{\cG}{\mathcal G}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cU}{\mathcal U}
\newcommand{\scrR}{\mathscr R}
\newcommand{\tcG}{\widetilde{\mathcal G}}

\newcommand{\pp}{\mbox{\egothfamily p}}

\newcommand{\ac}[1]{\actuarialangle{#1}}


%%Styles for bold symbols

\def\av{\boldsymbol a}
\def\bv{\boldsymbol b}
\def\cv{\boldsymbol c}
\def\dv{\boldsymbol d}
\def\ev{\boldsymbol e}
\def\fv{\boldsymbol f}
\def\gv{\boldsymbol g}
\def\hv{\boldsymbol h}
\def\iv{\boldsymbol i}
\def\jv{\boldsymbol j}
\def\kv{\boldsymbol k}
\def\lv{\boldsymbol l}
\def\mv{\boldsymbol m}
\def\nv{\boldsymbol n}
\def\ov{\boldsymbol o}
\def\pv{\boldsymbol p}
\def\qv{\boldsymbol q}
\def\rv{\boldsymbol r}
\def\sv{\boldsymbol s}
\def\tv{\boldsymbol t}
\def\uv{\boldsymbol u}
\def\vv{\boldsymbol v}
\def\wv{\boldsymbol w}
\def\xv{\boldsymbol x}
\def\yv{\boldsymbol y}
\def\zv{\boldsymbol z}
\def\Av{\boldsymbol A}
\def\Bv{\boldsymbol B}
\def\Cv{\boldsymbol C}
\def\Dv{\boldsymbol D}
\def\Ev{\boldsymbol E}
\def\Fv{\boldsymbol F}
\def\Gv{\boldsymbol G}
\def\Hv{\boldsymbol H}
\def\Iv{\boldsymbol I}
\def\Gv{\boldsymbol J}
\def\Kv{\boldsymbol K}
\def\Lv{\boldsymbol L}
\def\Mv{\boldsymbol M}
\def\Nv{\boldsymbol N}
\def\Ov{\boldsymbol O}
\def\Pv{\boldsymbol P}
\def\Qv{\boldsymbol Q}
\def\Rv{\boldsymbol R}
\def\Sv{\boldsymbol S}
\def\Tv{\boldsymbol T}
\def\Uv{\boldsymbol U}
\def\Vv{\boldsymbol V}
\def\Wv{\boldsymbol W}
\def\Xv{\boldsymbol X}
\def\Yv{\boldsymbol Y}
\def\Zv{\boldsymbol Z}


\def\Abf{\mathbf A}
\def\Bbf{\mathbf B}
\def\Cbf{\mathbf C}
\def\Dbf{\mathbf D}
\def\Ebf{\mathbf E}
\def\Fbf{\mathbf F}
\def\Gbf{\mathbf G}
\def\Hbf{\mathbf H}
\def\Ibf{\mathbf I}
\def\Gbf{\mathbf J}
\def\Kbf{\mathbf K}
\def\Lbf{\mathbf L}
\def\Mbf{\mathbf M}
\def\Nbf{\mathbf N}
\def\Obf{\mathbf O}
\def\Pbf{\mathbf P}
\def\Qbf{\mathbf Q}
\def\Rbf{\mathbf R}
\def\Sbf{\mathbf S}
\def\Tbf{\mathbf T}
\def\Ubf{\mathbf U}
\def\Vbf{\mathbf V}
\def\Wbf{\mathbf W}
\def\Xbf{\mathbf X}
\def\Ybf{\mathbf Y}
\def\Zbf{\mathbf Z}


\newcommand{\alphav}{\mbox{\boldmath{$\alpha$}}}
\newcommand{\betav}{\mbox{\boldmath{$\beta$}}}
\newcommand{\gammav}{\mbox{\boldmath{$\gamma$}}}
\newcommand{\deltav}{\mbox{\boldmath{$\delta$}}}
\newcommand{\epsilonv}{\mbox{\boldmath{$\epsilon$}}}
\newcommand{\zetav}{\mbox{\boldmath$\zeta$}}
\newcommand{\etav}{\mbox{\boldmath{$\eta$}}}
\newcommand{\iotav}{\mbox{\boldmath{$\iota$}}}
\newcommand{\kappav}{\mbox{\boldmath{$\kappa$}}}
\newcommand{\lambdav}{\mbox{\boldmath{$\lambda$}}}
\newcommand{\muv}{\mbox{\boldmath{$\mu$}}}
\newcommand{\nuv}{\mbox{\boldmath{$\nu$}}}
\newcommand{\xiv}{\mbox{\boldmath{$\xi$}}}
\newcommand{\omicronv}{\mbox{\boldmath{$\omicron$}}}
\newcommand{\piv}{\mbox{\boldmath{$\pi$}}}
\newcommand{\rhov}{\mbox{\boldmath{$\rho$}}}
\newcommand{\sigmav}{\mbox{\boldmath{$\sigma$}}}
\newcommand{\tauv}{\mbox{\boldmath{$\tau$}}}
\newcommand{\upsilonv}{\mbox{\boldmath{$\upsilon$}}}
\newcommand{\phiv}{\mbox{\boldmath{$\phi$}}}
\newcommand{\varphiv}{\mbox{\boldmath{$\varphi$}}}
\newcommand{\chiv}{\mbox{\boldmath{$\chi$}}}
\newcommand{\psiv}{\mbox{\boldmath{$\psi$}}}
\newcommand{\omegav}{\mbox{\boldmath{$\omega$}}}
\newcommand{\Sigmav}{\mbox{\boldmath{$\Sigma$}}}
\newcommand{\Lambdav}{\mbox{\boldmath{$\Lambda$}}}
\newcommand{\Deltav}{\mbox{\boldmath{$\Delta$}}}




\theoremstyle{plain}
\newtheorem{theo}{Theorem}[section]
\newtheorem{theorem}[theo]{Theorem}
\newtheorem*{theo*}{Theorem}      % unnumbered version
\newtheorem{lemma}[theo]{Lemma}
\newtheorem{propo}[theo]{Proposition}
\newtheorem{proposition}[theo]{Proposition}
\newtheorem{coro}[theo]{Corollary}
\newtheorem{corollary}[theo]{Corollary}



\theoremstyle{definition}
\newtheorem{defi}[theo]{Definition}
\newtheorem{definition}[theo]{Definition}
\newtheorem{conjecture}[theo]{Conjecture}
\newtheorem{claim}[theo]{Claim}
\newtheorem{problem}[theo]{Problem}

\theoremstyle{remark}
\newtheorem{remark}[theo]{Remark}
\newtheorem{exa}[theo]{Example}
\newtheorem{exe}[theo]{Exercise}
\newtheorem{pro}[theo]{Property}
\newtheorem*{solu*}{Solution}



